CodeJudge: Evaluating Code Generation with Large Language Models

Large Language Models (LLMs) have shown promising performance in code generation. However, how to reliably evaluate code generated by LLMs remains an unresolved problem. This paper presents CodeJudge, a code evaluation framework that leverages LLMs to evaluate the semantic correctness of generated code without the need for test cases. We investigate different ways to guide the LLM in performing "slow thinking" to arrive at an in-depth and reliable evaluation. We experimented with four LLMs as evaluators on four code generation datasets and five programming languages. The results show that CodeJudge significantly outperformed existing methods in most settings. Furthermore, compared with a SOTA GPT-3.5-based code evaluation method, CodeJudge achieved better results even when using a much smaller model, Llama-3-8B-Instruct. Our code and datasets are available on GitHub https://github.com/VichyTong/CodeJudge.

==> latex/sections/5_related_work.tex <==
\section{Related Works}
% We have described the existing code evaluation methods in Section \ref{sec: existing evaluation methods}. This section will mainly discuss ...

%\paragraph{\textbf{Code Generation Evaluation}} As detailed in Section \ref{sec: existing evaluation methods}, test-based methods such as the pass@k metric~\citep{chen2021evaluating} and EvalPlus~\citep{liu2023is} require human-made test cases. Most methods used in code generation evaluation are token-based~\citep{papineni-etal-2002-bleu,lin-2004-rouge,denkowski-lavie-2014-meteor,popovic-2015-chrf,8813269,ren2020codebleu}. Recently, explorations have been made into the embedding-based method, CodeBERTScore~\citep{zhou-etal-2023-codebertscore}, and the LLM-based method, ICE-Score~\citep{zhuo2023large}.

% \paragraph{\textbf{LLMs as Interpreters and Evaluators}}
% Our work is related to the topic of leveraging LLMs for roles in interpretation and evaluation, exploring their potential to revolutionize various domains. For example, in human-computer interaction, these models can provide useful feedback for UI design~\citep{10.1145/3586182.3615810}. Moreover, in the domain of computer vision, LLMs serve as interpreters for 3D layouts, enhancing the flexibility and interactivity of visual content creation~\citep{lin2023towards}. Our work focuses on leveraging the code interpretation abilities of LLMs, instructing LLMs as code interpreters to analyze code, identify mistakes, and categorize their severity. Finally, in NLP, there are efforts closely related to \citeeval{} that use LLMs as evaluators assigning correctness scores~\citep{fu2023gptscore,liu-etal-2023-g} or identify and categorize translation errors~\citep{perrella-etal-2022-matese,fernandes-etal-2023-devil}. 

% Some code ranking or code review models also have a component that locates or analyzes errors in generated code...\todo{Add citations and elaborate.}

\paragraph{LLMs for Code.}
General-purpose LLMs have utilized open-source code datasets for training in code generation and understanding tasks, achieving promising performances~\citep{10.5555/3648699.3648939,touvron2023llama,achiam2023gpt}. Additionally, models that are specifically tuned or fine-tuned for code-related tasks have demonstrated better performance compared to their comparable or even larger-sized general-purpose LLMs~\citep{chen2021evaluating,wang-etal-2021-codet5,li2022competition,li2023starcoder,rozière2023code}.
%\paragraph{Instruction-tuned Code LLMs.}

To improve the models' performance on unseen tasks, a fine-tuning method called Instruction~\citep{wei2022finetuned} tuning has been adapted for code generation, with many models being tuned or fine-tuned on datasets that include both natural language instructions and open-source programs~\citep{rozière2023code, shen2023pangu, wang-etal-2023-codet5, luo2024wizardcoder}. \citet{ma2024at} showed that instruction tuning can enhance both task-specific abilities and general reasoning capabilities. Our \citeeval{} using instruction-tuned models, such as CodeLlama-Instruct and GPT-3.5-Turbo, leverages the capability of these models to follow instructions and their reasoning abilities.


\paragraph{LLMs as feedback providers.}
Previous work has already highlighted that feedback from LLMs can provide valuable insights for humans in areas such as UI design \cite{10.1145/3586182.3615810} and 3D layouts \cite{lin2023towards}. Given the high costs and unreliability associated with human annotations in model training, researchers tried to use feedback from LLMs to aid human annotators \cite{saunders2022self} and directly train LLMs \cite{burns2023weak}. Moreover, \citet{NEURIPS2023_91edff07} demonstrated that feedback from certain LLMs can be used to iteratively refine the initial outputs from other LLMs.

% \paragraph{Code reranking methods.}
% Some code reranking methods aim to predict the correctness of generated code by leveraging neural models. \citet{yin-neubig-2019-reranking} developed a reranking model using both generative reconstruction features and discriminative matching features. \citet{10.5555/3618408.3620165} augments the code generation model to evaluate the likelihood of the instruction given the generated program, effectively using it as a ``reviewer'' model. More recently, \citet{pmlr-v202-ni23b} introduced a model that determines the correctness of a program based on the natural language input, the program itself, and its execution results. In comparison, \citeeval{} is a simpler method that requires neither training nor model conversion.

% Moreover, many code reranking methods also include a component that locates or analyzes errors in generated code. Many methods have been proposed to leverage execution-based output consistency to rerank generated programs~\citep{shi-etal-2022-natural, chen2023codet,zhang-etal-2023-self}, other methods leverage neural models to rerank generated programs~\citep{inala2022faultaware}. In particular, \citet{inala2022faultaware} creates a fault-aware ranker dataset that contains information about the program, its correctness, and the types of errors encountered, should there be any. This dataset is then utilized to fine-tune the CodeBERT model~\citep{feng-etal-2020-codebert}, which is augmented with an additional classification head and a line prediction head. Subsequently, this fine-tuned model is employed to predict various specific execution error types in the generated program. However, \citeeval{} does not require test cases and execution, which means our framework can be applied to more situations.


==> tables/combined_accuracy.tex <==
\begin{table}[ht]
\centering
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{l|c|c}
\hline
\textbf{Methods} & \textbf{HE-X} & \textbf{APPS} \\

\headercolorlong
\multicolumn{3}{c}{\textbf{CodeLlama-Instruct-34B}}\\
\tableskip
\bool{} & 62.93 & 40.00 \\
~~w/ \reference{} & 62.22 & 39.33  \\
\codedual{} & 71.52 & 56.33 \\
~~w/ \reference{} & 76.01 & 62.67 \\
\headercolorlong
\multicolumn{3}{c}{\textbf{Meta-Llama-3-8B-Instruct}}\\
\tableskip
\bool{} & 59.75 & 44.33 \\
~~w/ \reference{} & 55.10 & 43.33 \\
\codedual{} & 69.29 & 47.00 \\
~~w/ \reference{} & 72.22 & 53.00 \\
\headercolorlong
\multicolumn{3}{c}{\textbf{Meta-Llama-3-70B-Instruct}}\\
\tableskip
\bool{} & 77.37 & 55.67 \\
~~w/ \reference{} & 77.73 & 64.33 \\
\codedual{} & 81.67 & 68.00 \\
~~w/ \reference{} & 83.64 & 70.33 \\
\headercolorlong
\multicolumn{3}{c}{\textbf{GPT-3.5-Turbo-1106}}\\
\tableskip
\bool{} & 65.15 & 40.33 \\
~~w/ \reference{} & 75.96 & 52.67\\
\codedual{} & 73.13 & 57.00 \\
~~w/ \reference{} & 80.56 & 68.33 \\

\end{tabular}
}
\caption{Average accuracy (\%) across five programming languages in the binary classification task of the HumanEval-X dataset and accuracy of the APPS dataset.}
\label{tbl: combined accuracy}
\end{table}

